Ghost Value Augmentation for $k$-Edge-Connectivity

We give a poly-time algorithm for the $k$-edge-connected spanning subgraph ($k$-ECSS) problem that returns a solution of cost no greater than the cheapest $(k+10)$-ECSS on the same graph. Our approach enhances the iterative relaxation framework with a new ingredient, which we call ghost values, that allows for high sparsity in intermediate problems. Our guarantees improve upon the best-known approximation factor of $2$ for $k$-ECSS whenever the optimal value of $(k+10)$-ECSS is close to that of $k$-ECSS. This is a property that holds for the closely related problem $k$-edge-connected spanning multi-subgraph ($k$-ECSM), which is identical to $k$-ECSS except edges can be selected multiple times at the same cost. As a consequence, we obtain a $\left(1+O\left(\frac{1}{k}\right)\right)$-approximation algorithm for $k$-ECSM, which resolves a conjecture of Pritchard and improves upon a recent $\left(1+O\left(\frac{1}{\sqrt{k}}\right)\right)$-approximation algorithm of Karlin, Klein, Oveis Gharan, and Zhang. Moreover, we present a matching lower bound for $k$-ECSM, showing that our approximation ratio is tight up to the constant factor in $O\left(\frac{1}{k}\right)$, unless $P=NP$.

==> tex/algo_and_proof_nathan.tex <==
\section{Algorithm and Proof}

\begin{algorithm}[h]
\caption{}
\begin{algorithmic}[1]
\State Let $x$ be an extreme point solution to \eqref{eq:k_ecsmlp}
\While {$x$ is not integral}
\State If there is an edge $e$ with $x_e = 0$, delete it from $G$. For every edge $e$ with $x_e \ge 1$, add the constraint $\lfloor x_e \rfloor \le x_e \le \lceil x_e \rceil$ to the LP.
\If{there exists an edge $e=(u,v)$ such that $\frac{k}{2}-2 \le x_e < \frac{k}{2}$}
	\State Add the constraint $x_e \ge \frac{k}{2}$. 
\Else{}
	\State By \cref{thm:keytechnical} there exists a minimal constraint $S$ of the basis for $x$ with at most three fractional edges. Drop the constraint for $S$, all sets crossing $S$, and all subsets of $S$ in \eqref{eq:k_ecsmlp}. %Drop both!
\EndIf
\State Re-solve the LP to obtain a new extreme point solution $x$ to the updated set of constraints. 
\EndWhile 
\State By \cref{lem:wellconnected} the graph is $(k-5)$-edge-connected. Now add three spanning trees and min-cost matchings on the odd vertices of two of them to add a 5-edge-connected graph of cost at most $\frac{8}{k} \cdot c(x)$.
\end{algorithmic}
\label{alg-derand}
\end{algorithm}

We pay $\frac{8}{k} \cdot c(x)$ for the last fixing step and a factor of $\frac{4}{k-4}$ on the edges we increase from $\frac{k}{2}-2$ to $\frac{k}{2}$ (which clearly occurs at most once for each edge). The algorithm terminates in polynomial time as we ``make progress'' in every step: we either fix a new edge to at least $\frac{k}{2}$, drop a vertex constraint, or make the graph smaller (dropping all constraints crossing or contained in a set $S$ is equivalent to contracting it). So we get a $1+\frac{8}{k}+\frac{4}{k-4}$ approximation, or a $1+\frac{13}{k}$ approximation assuming $k \ge 20$. 

We call a family $\cL \subseteq 2^V$ laminar if no two sets cross. Two sets $S,T \subseteq V$ cross if $S \smallsetminus T, T \smallsetminus S, S \cap T, \overline{S \cup T}$ are all non-empty. Perhaps after taking complements, we may assume $\cL$ has the property that for all $S,T \in \cL$, we have $S \subseteq T$, $T \subseteq S$, or $S \cap T = \emptyset$. We call a set $S$ tight if $x(\delta(S)) = k$. 

We will use $\text{span}(\cL)$ to indicate the span of the constraints generated by sets in $\cL$.  

Our main theorem is as follows, which is an immediate consequence of the two lemmas after it (setting $\alpha = 2$):
\begin{theorem}\label{thm:keytechnical}
Let $x$ be an extreme point solution to \eqref{eq:k_ecsmlp} in which some  constraints with at most three fractional edges have been dropped and some constraints $x_e = \frac{k}{2}$ have been added, i.e., it is an LP solution seen while the above algorithm is running. Then, either there exists a pair of vertices $u,v$ with $\frac{k}{2} > \sum_{e \in E \mid e=\{u,v\}} x_e \ge \frac{k}{2}-2$, or there exists a set $S$ that is a minimal set in the basis of $x$ and has at most three fractional edges.
\end{theorem}

In the following we treat all dropped sets as contracted to simplify the exposition. 
\begin{lemma}\label{lem:keytechnicaluncrossing}
	Let $x \in \R^{E}$ be fractional vector such that for all $S \subseteq V$ with $2 \le |S| \le n-2$, $x(\delta(S)) \ge k$, and for all $S \subsetneq V$ with $S\neq \emptyset$, $x(\delta(S)) \ge k-\alpha$. 
	
	Let $\cF \subseteq 2^V$ be the family of tight sets $S$ with $2 \le |S| \le n-2$. Then, either:
	\begin{enumerate}
		\item There exists a laminar family $\cL$ of tight sets such that $\text{span}(\cL) = \text{span}(\cF)$, or %where F is the set of sets that have not been dropped!
		\item There exists an edge $e$ such that $\frac{k}{2} > x_e \ge \frac{k}{2}-\alpha$.  
	\end{enumerate}
\end{lemma}
\begin{proof}
	Let $\cL$ be any maximal laminar family of tight sets such that $\text{span}(\cL) \subseteq \text{span}(\cF)$. Now, suppose that there exists $T \in \cF$ such that $T \not\in \text{span}(\cL)$. It must cross some set in $\cL$. Find a set $T \not\in \text{span}(\cL)$ which crosses the minimal number of sets in $\cL$, and let $S$ be an arbitrary set it crosses in $\cL$. If no such set exists, then (1) holds and we are done.
	
	First assume $x(\delta(S \cap T)) \ge k$; we will get a contradiction. We have
		$$2k = x(\delta(S)) + x(\delta(T)) = x(\delta(S \cup T)) + x(\delta(S \cap T)) + 2x(E(S \smallsetminus T, T \smallsetminus S)).$$
		But since $x(\delta(S \cap T)) \ge k$ and $x(\delta(S \cup T)) \ge k$ (as $|S \cup T| \ge 2$), it must be that $x(\delta(S \cap T)) = x(\delta(S \cup T)) = k$ and $E(S \smallsetminus T, T \smallsetminus S) = \emptyset$. We have:
		$$\chi(\delta(T)) = \chi(\delta(S \cap T)) + \chi(\delta(S \cup T)) - \chi(\delta(S))$$
		 Since $S \cap T \subseteq T$ and $T$ crossed the minimal number of sets, it must be that $\chi(\delta(S \cap T)) \in \text{span}(\cL)$. So, it must be that $\chi(\delta(S \cup T)) \not\in \text{span}(\cL)$. However, one can check that every set crossing $S \cup T$ in $\cL$ must also cross $T$, as $S$ is not crossed in $\cL$. Thus since $T$ is also crossed by $T$, by minimality of the number of sets crossing $T$ we get a contradiction. 

So it must be that $x(\delta(S \cap T)) < k$ which by the assumption of the lemma implies $|S \cap T| = 1$. If $x(\delta(S \smallsetminus T)) \ge k$ and $x(\delta(T \smallsetminus S)) \ge k$, then using a similar uncrossing step we get a contradiction. So it must be that at least one of these two sets, say $S \smallsetminus T$, has $x(\delta(S \smallsetminus T)) < k$ (the other case is similar), which implies $|S \smallsetminus T| = 1$. Let $u = S \smallsetminus T$ and $v = S \cap T$. So, $x(\delta(v)), x(\delta(u)) \ge k-\alpha$ and $x(\delta(S)) = k$. This gives:
$$2k-2\alpha \le x(\delta(u)) + x(\delta(v)) = x(\delta(S)) + 2x_e,$$
which implies $x_e \ge \frac{k}{2}-\alpha$. Similarly we have
$$2k > x(\delta(u)) + x(\delta(v)) = x(\delta(S)) + 2x_e = k+2x_e,$$
which implies $x_e < \frac{k}{2}$.
\end{proof}


\begin{lemma}\label{lem:keytechnicallaminar}
Let $\cL \subseteq 2^{V}$ be a laminar family of tight sets for an LP solution $x$ to \eqref{eq:k_ecsmlp} (which may have some constraints dropped and some box constraints added) which together with the box constraints form a linearly independent system spanning all tight constraints of $x$. Then, some minimal constraint $S$ in $\cL$ has at most three fractional edges. 	
\end{lemma}
\begin{proof}
	Suppose not, and there are at least 4 fractional edges in $\delta(S)$ for every minimal constraint $S \in \cL$. 
		
	Let $\ell$ be the number of edges $e$ with $x_e \not\in \Z$. We will use a token counting argument to show that $\ell < |\cL|$, which is a contradiction. To do so, we will assign 2 tokens to every edge and show that there is an assignment of tokens to sets in $\cL$ such that every set gets at least 2 tokens and at least one token is left over.  
	
	 Let every fractional edge $e=(u,v)$ assign a token to the smallest set in $\cL$ containing $u$ and a token to the smallest set in $\cL$ containing $v$. In this way, every minimal set in $\cL$ gets at least 4 tokens. We will inductively show that every set can keep 2 tokens and give 2 tokens to its parent. Thus, every maximal set in $\cL$ will receive 4 tokens. In this way, we show that $2\ell < 2|\cL|$ (since there is at least one maximal set), contradicting that $x$ is an extreme point solution.  
	
	For the base case, we know every minimal set has at least 4 fractional edges, thus we are done. So, let $S \in \cL$ be a non-minimal set. If $S$ has 2 or more tight children then we receive 4 tokens from our children and we are done. Otherwise, $S$ has a single tight child $S'$. But then, where $F$ is the set of fractional edges, $(\delta(S)\cap F) \not= (\delta(S') \cap F)$ since they are linearly independent with each other and the box constraints.  Since $x(\delta(S) \cap F),x(\delta(S') \cap F)$ are integers, we must have $|(\delta(S)\cap F) \Delta (\delta(S)\cap F)| \ge 2$. However, observe that every $e \in (\delta(S)\cap F) \Delta (\delta(S)\cap F)$ has an endpoint in $S \smallsetminus S'$. But then each such edge gives a token to $S$. So, we receive 2 tokens from our child $S'$ and 2 tokens from the (at least two) edges in $(\delta(S)\cap F) \Delta (\delta(S)\cap F)$ as desired and can keep 2 and give 2 to the parent of $S$. 
\end{proof}

The condition of the next lemma (integrality of $E(S)$) is met by a leaf of an extreme point as there are no tight (non-box) constraints contained inside of it.

\begin{lemma}\label{lem:wellconnected}
Let $\alpha$ be an even integer. Let $S$ be a set with at most $\alpha+1$ fractional edges and for which $E(S)$ is integral. Let $x \in \R^{E}$ as in \cref{lem:keytechnicaluncrossing}. Let $T$ be any set crossing $S$ or contained in $S$. Then, if $G/S$ is $k-\alpha$-edge-connected by a solution $R \subseteq E$ and the box constraints on $x$ are met by $R$, then $|\delta(T) \cap (R \cup E(S))| \ge k-\frac{5}{2}\alpha$.
\end{lemma}
\begin{proof}
	Let $R^* = R \cup E(S)$. First consider the case in which $T \subseteq S$. If $T$ was dropped previously then there is nothing to be done. Otherwise at most $\alpha+1$ edges in $\delta(T)$ are not integral since all of them must be in $\delta(S)$, so clearly $|\delta(T) \cap R^*| \ge k-\alpha$ since $x(\delta(T)) \ge k$.
	
	Otherwise, $T$ crosses $S$. Let $\ell = x(\delta(T) \cap E(S)) = |\delta(T) \cap E(S)|$. We have:	
	$$2k-2\alpha \le x(\delta(T \cap S)) + x(\delta(S \smallsetminus T)) = x(\delta(S)) + 2\ell = k+2\ell$$
	Therefore, $\ell \ge \frac{k}{2}-\alpha$.  
	
	Let $m = x(\delta(T \smallsetminus S) \cap \delta(S)) \ge \frac{k}{2}-\alpha$. We have (using that $T \cup S$ has not yet been dropped, however note $T \smallsetminus S$ may have been dropped):
	$$2k-\alpha \le x(\delta(T \smallsetminus S)) + x(\delta(T \cup S)) = x(\delta(S)) + 2m = k+2m$$
	So $m \ge \frac{k-\alpha}{2}$. Of the set of edges comprising $m$, at most $\alpha+1$ are fractional since they are all in $\delta(S)$. Thus there are at least $\frac{k-\alpha}{2}-\alpha$ integral ones in $R^*$. So there are at least $\frac{k}{2}-\alpha + \frac{k-\alpha}{2}-\alpha = k - \frac{5}{2}\alpha$ edges in $\delta(T) \cap R^*$. 
\end{proof}


==> tex/conclusion.tex <==
\section{Conclusion}
\todoeh{We should make sure we write a conclusion or delete it}
